Nonet at SemEval-2023 Task 6: Methodologies for Legal Evaluation

This paper describes our submission to the SemEval-2023 for Task 6 on LegalEval: Understanding Legal Texts. Our submission concentrated on three subtasks: Legal Named Entity Recognition (L-NER) for Task-B, Legal Judgment Prediction (LJP) for Task-C1, and Court Judgment Prediction with Explanation (CJPE) for Task-C2. We conducted various experiments on these subtasks and presented the results in detail, including data statistics and methodology. It is worth noting that legal tasks, such as those tackled in this research, have been gaining importance due to the increasing need to automate legal analysis and support. Our team obtained competitive rankings of 15$^{th}$, 11$^{th}$, and 1$^{st}$ in Task-B, Task-C1, and Task-C2, respectively, as reported on the leaderboard.

==> files/anup_model.tex <==
For L-NER, we propose an innovative approach that leverages the strengths of pre-trained transformer models and domain-specific embeddings to build custom NER models in the legal domain. Specifically, our model architecture involves fine-tuning a RoBERTa ~\cite{liu2019roberta} transformer with Spacy\footnote{https://spacy.io/} and incorporating external embeddings from Law2Vec\footnote{https://archive.org/download/Law2Vec} (200 dimensions) to enhance the corpus's contextual understanding of legal terms.

Our pipeline involves data preparation, pipeline configuration, model fine-tuning, and evaluation. To begin with, we use the dataset provided by the organizers and create Doc objects that contain the text. We also incorporate external embeddings from Law2Vec to enhance the corpus's contextual understanding of legal terms. The custom Spacy's model training procedure is shown in Figure~\ref{fig:Spacy Training Procedure}\footnote{https://spacy.io/usage/training/}, which involves an iterative process of comparing the model's predictions against reference annotations to estimate the gradient of the loss and using it to calculate the gradient of the weights through back-propagation. The gradients indicate how the weight values should be changed so that the model’s predictions become more similar to the reference labels over time.

\begin{figure}[h]
  \includegraphics[width=\linewidth]{images/spacy.png}
  \caption{Spacy Custom NER Training Procedure }
  \label{fig:Spacy Training Procedure}
\end{figure}
\FloatBarrier

The Spacy pipeline configuration includes the RoBERTa transformer model, the Law2Vec embeddings, and additional NER components using the transformer, ner, and vectors components provided by Spacy. We fine-tune the BERT transformer model with the Adam.V1 optimization algorithm, a learning rate of $2e^{-5}$, and 100 epochs, and evaluate the performance of our model on a separate test set.
SpaCy Model description in detail is here\footnote{https://tinyurl.com/SpaCy-Model-description}. SpaCy is powerful but somewhat opaque and hard to modify.
Overall, our work demonstrates the effectiveness of our model architecture for fine-tuning BERT transformers with Spacy 3 for Legal NER and highlights the potential of incorporating external embeddings from Law2Vec for building high-performance NER models in the legal domain.


==> files/ayush_model.tex <==
We perform the task of Named Entity Recognition for legal documents using a pre-trained legal BERT base uncased model~\cite{chalkidis-etal-2020-legal}. The model architecture comprises a BERT model with a token-level classifier, followed by a Linear-Chain CRF. \\
For an input sequence of n tokens, BERT outputs an encoded token sequence with hidden dimension H. The classification model takes each token's encoded representation to the tag space, i.e., $\mathbb{R}^H$ -> $\mathbb{R}^K$, where $K$ is the number of tags in the dataset. And the output score maps to $\mathbb{R}^{n*K}$ of the classification model which is then fed to the CRF layer, which is used to predict in BIO format.\\
When we tested on BERT-CRF, our model could have performed better in this way because the sentence length was too much and the number of entities significantly less. Even in some of the training sentences, there were no entities in the sentence. We tried to make it more robust by adding part of the speech tag in the embedding layer of the BERT model. The observation behind providing further Embedding is that most of the named entities are nouns, so we want our span to be more exact.\\
In the classical BERT model ~\cite{devlin-etal-2019-bert}, we have input embeddings as the sum of the token embeddings, the segment embedding, and the position embedding. After getting input embedding, it passes to Bert Layer Norm, then the dropout layer. After that, we return to the Embedding.\\
Actually, we cannot directly append a POS tag with the token because the pre-trained tokenizer only knows the token, not the token + POS tags. A better way is to create an additional input to the model(besides input\_ids and token\_type\_ids) called pos\_tags\_ids, for which we add an additional embedding layer(nn. Embedding) ~\ref{fig:Modified BERT Embedding Layer}. In that way, we sum the Token embeddings, token types, and POS tags. The max number of a pos tag is the total unique number of POS tags, also called the "vocabulary size" of the embedding layer. The hidden size is the size of the embedding vector that we want to learn for each pos tag(which is 768 by default for BERT-base). 
In order to improve the performance of the BERT-CRF model for named entity recognition (NER), we have generated part-of-speech (POS) tags as an additional feature for the provided dataset. These tags are used in conjunction with the tokens during training to make NER tag predictions. The POS tags are generated for each token in the sentences using a pre-trained spaCy~\cite{spacy2} model, which has demonstrated an accuracy of 97\%\footnote{https://spacy.io/usage/facts-figures} for this specific task.  

An additional complexity of BERT-like models is that they rely on subword tokens, rather than words. This means that a word like "playing" might be tokenized into ["play", "\#\#ing"]. This means that we will also have to provide POS tags at the token level. Similar to how each token is turned into an integer (input\_ids), we will also have to turn each POS tag into a corresponding integer (pos\_tag\_ids) in order to provide it to the model. So we would actually need to keep a dictionary that maps each POS tag to a corresponding integer.

\begin{figure}[h]
  \includegraphics[width=\linewidth]{images/new_BERT.png}
  \caption{Modified BERT Embedding Layer}
  \label{fig:Modified BERT Embedding Layer}
\end{figure}


==> files/shubham_model.tex <==
As discussed above, two models were trained to perform legal name entity recognition task. These models are SPACY and BERT-CRF. The output of both models is an array of tuples consisting of the entity's starting index, ending index, and label. To determine the final prediction, if the tuples in the output of both models intersect (start, end), then the intervals are merged, keeping the label the same for the final prediction. For instance, if the prediction from the SPACY model is (43,53, ORG) and that of the BERT-CRF model is (45,60, ORG), the final output will be (43,60, ORG). Otherwise, the union of outputs is taken from both models. This approach improved the prediction accuracy by 2\% compared to using only the SPACY model for this task.


\begin{figure}[h]
  \includegraphics[width=\linewidth]{latex/images/Diagram3.png}
  \caption{Fusion of Models}
  \label{fig:models_fusion}
\end{figure}
\FloatBarrier




==> files/todo.tex <==
\begin{itemize}

  \item We solved the subtask-B Legal Named Entity Recognition. Legal NER takes the first step in extracting relevant entities for retrieval and information extraction. There are various entities in the legal domain namely names of petitioner, respondent, court, statute, precedent, etc which are detected by the Legal-NER system developed specifically for Indian Court cases.
  
  \item We solved the subtask-C namely Legal Judgement prediction with explanation. The task is a binary classification task to detect whether the decision of the legal case is in favour of the appellant or defendant. Also there is a explanation which tries to determine the reasoning behind the decision of the legal case. The system gives a decision along with an explanation for a legal case specifically designed for Indian Court cases. We solved both subtask C1, Legal Judgement Prediction and subtask C2, Court Judgement Prediction with explanation. 


  
    %\item Introduction should have the each task description
    %\item Each section should have subsections for each sub-tasks
\end{itemize}




